Erlang Code Evolution Control

During the software lifecycle, a program can evolve several times for different reasons such as the optimisation of a bottle-neck, the refactoring of an obscure function, etc. These code changes often involve several functions or modules, so it can be difficult to know whether the correct behaviour of the previous releases has been preserved in the new release. Most developers rely on a previously defined test suite to check this behaviour preservation. We propose here an alternative approach to automatically obtain a test suite that specifically focusses on comparing the old and new versions of the code. Our test case generation is directed by a sophisticated combination of several already existing tools such as TypEr, CutEr, and PropEr; and other ideas such as allowing the programmer to chose an expression of interest that must preserve the behaviour, or the recording of the sequences of values to which this expression is evaluated. All the presented work has been implemented in an open-source tool that is publicly available on GitHub.

==> Secciones/unused.tex <==
%!TEX root = ../paper.tex

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Ideas and techniques to reduce program slices}
\label{sec_ideas}

There are several ideas that we could use to reduce the size of a slice. In this section, we show that none of these ideas can produce a minimal slice by themselves, and thus, we have to study how to combine them to exploit their synergies. 

\bigskip
\noindent{\bf Slicing slices}. 
Different program slicers usually implement different techniques and optimizations to further reduce the size of a slice. Hence, we can use an already existing program slicer to produce a first slice that we can use as the starting point to further reduce its size with another program slicer. The slice of a slice is a slice if the same slicing criterion is used: 

\begin{theorem} 
\label{theo-slice}
Let $P$ be a program, and $S=slice_X(P,C)$ be a program slice.
Then, $slice_Y(S,C) \in \cS lices_C^P$ for any $X$, $Y$, and $C$.
\end{theorem}

\begin{proof}
By point 1 in Definition~\ref{def_Slice}, we know that $S' \subseteq S \subseteq P$. 
By point 2 in Definition~\ref{def_Slice}, we know that $P$, $S$, and $S'$ compute the same values for $C$. 
Hence, $S' \in \cS lices_C^P$.
\end{proof}

%
%We could reduce slices combining two or more slicers. For instance, 
Hence, given a program P, $slice_A(slice_B(P))$ could take advantage of the combined power of the slicers $A$ and $B$. Unfortunately, this would produce a local minimum. In fact, assuming that these slicers are reliable, this would produce a reduced complete slice, but it could be still incorrect (i.e., it could contain a line of code that is retained by all the slicers but it does not affect the slicing criterion). 

\bigskip
\noindent{\bf Observation-Based Slicing (ORBS)}. It is a technique that allows for removing a part of the program, and use testing to check whether the remaining part behaves as expected~\cite{BinGHI14}. 
%JJJ: It uses a shrinking process similar to other tools such as QuickCheck and PropER
Hence, we can use ORBS to check whether all parts of the program are actually needed by incrementally removing all parts. 
%
Here again, the confidence of ORBS depends on the quality of the test cases. Thus, we cannot guarantee completeness with this method.

\bigskip
\noindent{\bf Testing}. 
There exist methods to compute slices that are not complete (e.g., Critical Slicing~\cite{DeMPS96} and Delta Debugging~\cite{CleZ00,ZelH02}). We can use test case generation to compare the behaviour of the original program and its slices. If the observable behaviour is different for a test case, this means that the slice is not a proper slice (according to Definition~\ref{def_Slice}), often because the slice is not complete (i.e., a statement needed is missing, which produced a wrong value in the slicing criterion). 
%
Of course, testing is not a guarantee that a slice is complete, because full path coverage is undecidable; but it is a powerful tool to automatically discard false positives, and it also provides help in the manual inspection of slices. 


\bigskip
\noindent{\bf Fine-grain slices}. Program slices have traditionally been measured in code lines. The reason is that most program slicing techniques consider the code lines as atomic elements and, thus, they remove a whole line or nothing~\cite{Wei81,DeMPS96,BinGHI14}. 
For this reason, most of the work that compares the precision of different program slicing techniques just compare the retrieved number of lines (see, e.g.,~\cite{BinGH07,BinGHI14}). 
Unfortunately, this is very sensitive to the programming style, and moreover, it can be very imprecise, especially in functional languages.

\begin{example}
\label{ex_running}
Consider the Erlang program in Figure~\ref{fig_EDG} (top-left) and its minimal slice (top-right) with respect to the slicing criterion {\tt (10,B)}. 
Observe that some expressions have been replaced with {\tt \_} or with the fresh atom {\tt undef}. This is needed to make the slice executable. 
Clearly, all methods based on lines will not be able to remove the subexpressions that are not needed at lines 1, 2, 3 and 6. 
For instance, at line 2, {\tt C=B} can be removed, but the programmer initialized {\tt A}, {\tt B} and {\tt C} in a single line, and thus the whole line cannot be removed.
One can argue that a preprocessing phase could be used to refactor the code and place all statements in different lines whenever it is possible. 
But this cannot solve the second problem: sometimes only a subexpression can be removed in a line. This is the case of variables {\tt Z}, {\tt Y}, and {\tt C} at line 3.  

\begin{figure}

{\em
\begin{center}
$~~~~~~~~~~~~~~~~~~~$
\begin{minipage}[t]{0.40\textwidth}
Original Program
\lstset{language = erlang, basicstyle=\ttfamily\scriptsize}
\lstset{numbers=left, stepnumber=1, numberstyle=\scriptsize}
\begin{lstlisting}
main(X,Y) ->
  A=1, B=A, C=B,
  Z=foo(X,{Y,B,C}),
  Z.

foo(X,{Y,B,C}) ->  
  case X of		 
    123456789 -> Z=X/Y,
                 Z+C; 
    2         -> B;
    _         -> 42
  end.
\end{lstlisting}
\end{minipage}
$~~~~~~~$
\begin{minipage}[t]{0.40\textwidth}
Minimal Slice for {\tt (10,B)}
\lstset{language = erlang, basicstyle=\ttfamily\scriptsize}
\lstset{numbers=left, stepnumber=1, numberstyle=\scriptsize}
\begin{lstlisting}
main(X,_) ->
  A=1, B=A,
  _=foo(X,{undef,B,undef}).


foo(X,{_,B,_}) ->  
  case X of		 


    2 -> B	

    end.
\end{lstlisting}
\end{minipage}\\
$~$ Erlang Dependence Graph $~$\\
\includegraphics[scale = 0.27]{\figures{EDG.jpg}}
\end{center}
}

\caption{Erlang program, its minimal slice, and the EDG associated with line 2}
\label{fig_EDG}

\end{figure}
\end{example}

In this paper we propose to use the nodes of the abstract syntax tree that represents the program as the minimum information unit that can be sliced. In the case of the EDG this is absolutely precise, because the EDG represents every single literal in the program with a unique node. For instance, the EDG in Figure~\ref{fig_EDG} (down) represents the pattern matching statements at line 2. Variable {\tt C} is represented with a single (sliceable) node. 

If we use the EDG nodes as the measure unit to compare slices, we can be fully precise and distinguish slices such as the following (the underlining represents the parts of the code that can be removed):

\lstset{
  language=erlang, 
  basicstyle=\ttfamily\small, 
  moredelim=[is][\underbar]{_}{_}
}

\begin{lstlisting}[keepspaces=true]
_{A,B}={f(1,2),3}_    {A,_B_}={f(1,2),_3_}     {A,B}={f(_1_,2),3}     {A,B}={_f_(1,2),3}    
\end{lstlisting}

\noindent Contrarily, using the standard approach (based on lines), nothing would be removed in the four cases since there are expressions that cannot be removed. 
%statement on the left would be removed (as with the EDG), and the other statements would remain untouched (these lines cannot be removed). 
%
Due to its beneficial properties, in the following we will measure slices using EDG nodes. 

